Conservative Filtering for Heterogeneous Decentralized Data Fusion in Dynamic Robotic Systems

This paper presents a method for Bayesian multi-robot peer-to-peer data fusion where any pair of autonomous robots hold non-identical, but overlapping parts of a global joint probability distribution, representing real world inference tasks (e.g., mapping, tracking). It is shown that in dynamic stochastic systems, filtering, which corresponds to marginalization of past variables, results in direct and hidden dependencies between variables not mutually monitored by the robots, which might lead to an overconfident fused estimate. The paper makes both theoretical and practical contributions by providing (i) a rigorous analysis of the origin of the dependencies and and (ii) a conservative filtering algorithm for heterogeneous data fusion in dynamic systems that can be integrated with existing fusion algorithms. This work uses factor graphs as an analysis tool and an inference engine. Each robot in the network maintains a local factor graph and communicates only relevant parts of it (a sub-graph) to its neighboring robot. We discuss the applicability to various multi-robot robotic applications and demonstrate the performance using a multi-robot multi-target tracking simulation, showing that the proposed algorithm produces conservative estimates at each robot.

==> Figures/Full_graph_fig_backup.tex <==
\begin{figure*}[tb]
%\resizebox{3.4in}{1.6in}{%
\begin{tikzpicture}[ new set=import nodes]
 \begin{scope}[nodes={set=import nodes}]
      
      \node (a) at (-0.5,2.5) {$(a)$};
      \node (x_Li)[latent, minimum size=31pt] at (0,0) {$\chi^i_L$};
      \node (x_Lm)[latent,dashed, minimum size=31pt] at (0.5,2.25) {$\chi^m_L$};
      \node (x_Lj)[latent,dashed, minimum size=31pt] at (0.5,-2.25) {$\chi^j_L$};
      %\node (s2)[latent, dashed] at (0,-0.75) {$s_j$};
      \node [latent, right=of x_Li, yshift=+1.5cm, minimum size=31pt] (x_im) {$\chi^{im\setminus j}_{C,1}$};
      \node [latent, right=of x_Li, yshift=0, minimum size=31pt] (x_ijm) {$\chi^{ijm}_{C,1}$};
      \node [latent, right=of x_Li, yshift=-1.5cm, minimum size=31pt] (x_ij) {$\chi^{ij\setminus m}_{C,1}$};
      %\node [factor, right=of x1, label={$f(x_2|x_1)$}] (f1) {};
     % \node [latent, right=of f1, xshift=-0.55cm] (x2) {$x_2$};
      \node [factor, between=x_Li and x_im ] (yi11) {};
      \node [factor, between=x_Li and x_ijm ] (yi21) {};
      \node [factor, between=x_Li and x_ij ] (yi31) {};
     
      \node [factor, between=x_im and x_ijm ,label=right:$f^{im}_1$] (f_im) {};
      \node [factor, between=x_ij and x_ijm ,label=right:$f^{ij}_1$] (f_ij) {};
     
     \node [factor, right=of x_im,  label={$f^{im}_{2|1}$}] (f2_im) {};
      \node [latent, right=of f2_im, xshift=-0.55cm, minimum size=31pt] (x2_im) {$\chi^{im\setminus j}_{C,2}$};
      
      \node [factor, right=of x_ijm,   label={$f^{ijm}_{2|1}$}] (f2_ijm) {};
      \node [latent, right=of f2_ijm, xshift=-0.55cm, minimum size=31pt] (x2_ijm) {$\chi^{ijm}_{C,2}$};
      
      \node [factor, right=of x_ij, label={$f^{ij}_{2|1}$}] (f2_ij) {};
      \node [latent, right=of f2_ij, xshift=-0.55cm, minimum size=31pt] (x2_ij) {$\chi^{ij\setminus m}_{C,2}$};
      
      \node [factor,fill=black!40, between=x_Lj and x_ijm] (f_j11) {};
      \node [factor,fill=black!40, between=x_Lj and x_ij] (f_j21) {};
      
      \node [factor,fill=black!40, between=x_Lm and x_ijm] (f_m11) {};
      \node [factor,fill=black!40, between=x_Lm and x_im] (f_m21) {};
      
      %%%%%%%% (b) %%%%%%%%%%%%%%%%%%%%%%%%%%%
      
      \node (b) at (5.5,2.5) {$(b)$};
      \node (x_Lib)[latent, minimum size=31pt] at (6,0) {$\chi^i_L$};
      \node (x_Lmb)[latent,dashed, minimum size=31pt] at (6.5,2.25) {$\chi^m_L$};
      \node (x_Ljb)[latent,dashed, minimum size=31pt] at (6.5,-2.25) {$\chi^j_L$};

      %\node [factor, right=of x1, label={$f(x_2|x_1)$}] (f1) {};
     % \node [latent, right=of f1, xshift=-0.55cm] (x2) {$x_2$};
      \node [latent, right=of x_Lib, xshift=0.0cm, minimum size=31pt] (x2_ijmb) {$\chi^{ijm}_{C,2}$};
      
      \node [latent, above=of x2_ijmb, yshift=-0.5cm, minimum size=31pt] (x2_imb) {$\chi^{im\setminus j}_{C,2}$};
      
      \node [latent, below=of x2_ijmb, yshift=0.5cm, minimum size=31pt] (x2_ijb) {$\chi^{ij\setminus m}_{C,2}$};
     
     \node [factor,fill=red!100, between=x_Lib and x2_ijmb ] (f2b) {};
      
      %%%%%%%%%%%% (c) %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      \node (c) at (9.25,2.5) {$(c)$};
      \node (x_Lic)[latent, minimum size=31pt] at (9.75,0) {$\chi^i_L$};
      \node (x_Lmc)[latent,dashed, minimum size=31pt] at (10.25,2.25) {$\chi^m_L$};
      \node (x_Ljc)[latent,dashed, minimum size=31pt] at (10.25,-2.25) {$\chi^j_L$};

      %\node [factor, right=of x1, label={$f(x_2|x_1)$}] (f1) {};
     % \node [latent, right=of f1, xshift=-0.55cm] (x2) {$x_2$};
      \node [latent, right=of x_Lic, xshift=0.0cm, minimum size=31pt] (x2_ijmc) {$\chi^{ijm}_{C,2}$};
      
      \node [latent, above=of x2_ijmc, yshift=-0.5cm, minimum size=31pt] (x2_imc) {$\chi^{im\setminus j}_{C,2}$};
      
      \node [latent, below=of x2_ijmc, yshift=0.5cm, minimum size=31pt] (x2_ijc) {$\chi^{ij\setminus m}_{C,2}$};
     
     \node [factor,fill=red!100, between=x_Lic and x2_ijmc ] (f2c) {};
     
     %%%%%%%%%%%% (d) %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      \node (d) at (13,2.5) {$(d)$};
      \node (x_Lid)[latent, minimum size=31pt] at (13.5,0) {$\chi^i_L$};
      \node (x_Lmd)[latent,dashed, minimum size=31pt] at (14,2.25) {$\chi^m_L$};
      \node (x_Ljd)[latent,dashed, minimum size=31pt] at (14,-2.25) {$\chi^j_L$};

      %\node [factor, right=of x1, label={$f(x_2|x_1)$}] (f1) {};
     % \node [latent, right=of f1, xshift=-0.55cm] (x2) {$x_2$};
      \node [latent, right=of x_Lid, xshift=0.0cm, minimum size=31pt] (x2_ijmd) {$\chi^{ijm}_{C,2}$};
      
      \node [latent, above=of x2_ijmd, yshift=-0.5cm, minimum size=31pt] (x2_imd) {$\chi^{im\setminus j}_{C,2}$};
      
      \node [latent, below=of x2_ijmd, yshift=0.5cm, minimum size=31pt] (x2_ijd) {$\chi^{ij\setminus m}_{C,2}$};
     
     \node [factor,fill=red!100, between=x2_ijmd and x2_imd, label=right:\textcolor{red!100}{{$\tilde{f}^{im}_{2}$}} ] (f2d_im) {};
     \node [factor,fill=red!100, between=x2_ijmd and x2_ijd, label=right:\textcolor{red!100}{{$\tilde{f}^{ij}_{2}$}} ] (f2d_ij) {};
      
  \end{scope}
  
 \graph {
    (import nodes);
   
    % dynamic
    
    %{s3,x3}--f2, s4--[dashed]f2,
   
   % (b)
    {x_im,x_Li}--yi11, 
    {x_ijm,x_Li}--yi21,  
    {x_ij,x_Li}--yi31,
    {x_ij,x_ijm}--f_ij,
    {x_im,x_ijm}--f_im,
    {x2_ij,x_ij}--f2_ij,
    {x2_im,x_im}--f2_im,
    {x2_ijm,x_ijm}--f2_ijm,
    {x_Lm}--[dashed]f_m21, 
    {x_Lm}--[dashed]f_m11,
    {x_Lj}--[dashed]f_j21, 
    {x_Lj}--[dashed]f_j11,
    {x_im}--f_m21,
    {x_ijm}--f_m11,
    {x_ij}--f_j21, 
    {x_ijm}--f_j11,
    {x_Lib,x2_imb, x2_ijb, x2_ijmb }--f2b,
    {x_Ljb,x_Lmb}--[dashed]f2b,
    {x2_imc, x2_ijc, x2_ijmc }--f2c,
    {x2_ijmd, x2_imd}--f2d_im,
    {x2_ijmd, x2_ijd}--f2d_ij
    };
    
\end{tikzpicture}
\caption{Full graph perspective   }
      \label{fig:fullGraph_backup}
\end{figure*}

==> Figures/ProblemStatement_fig.tex <==
\begin{figure}[tb]
%\resizebox{3.4in}{1.6in}{%
\begin{tikzpicture}[ new set=import nodes]
 \begin{scope}[nodes={set=import nodes}]
      
      \node (a) at (-1,2) {$(a)$};
      \node (x_L)[latent, minimum size=31pt] at (-0.75,0) {$\chi^i_L$};
      %\node (s2)[latent, dashed] at (0,-0.75) {$s_j$};
      \node [latent, right=of x_L, yshift=1.5cm, minimum size=31pt] (x_im) {$\chi^{im\setminus j}_{C,1}$};
      \node [latent, right=of x_L, yshift=0, minimum size=31pt] (x_ijm) {$\chi^{ijm}_{C,1}$};
      \node [latent, right=of x_L, yshift=-1.5cm, minimum size=31pt] (x_ij) {$\chi^{ij\setminus m}_{C,1}$};
      %\node [factor, right=of x1, label={$f(x_2|x_1)$}] (f1) {};
     % \node [latent, right=of f1, xshift=-0.55cm] (x2) {$x_2$};
      \node [factor, between=x_L and x_im ,label=$f^{i,1}_{1}$] (yi11) {};
      \node [factor, between=x_L and x_ijm ,label=$f^{i,2}_{1}$] (yi21) {};
      \node [factor, between=x_L and x_ij ,label=$f^{i,3}_{1}$] (yi31) {};
      %\node [factor,fill=black!50, between=x1 and s2 ,label=below:$y^j_{1}$] (yj1) {};
      
      \node (b) at (2.25,2) {$(b)$};
      \node (x_Lb)[latent, minimum size=31pt] at (2.65,0) {$\chi^i_L$};
      %\node (s2)[latent, dashed] at (0,-0.75) {$s_j$};
      \node [latent, right=of x_Lb, yshift=+1.5cm, minimum size=31pt] (x_imb) {$\chi^{im\setminus j}_{C,1}$};
      \node [latent, right=of x_Lb, yshift=0, minimum size=31pt] (x_ijmb) {$\chi^{ijm}_{C,1}$};
      \node [latent, right=of x_Lb, yshift=-1.5cm, minimum size=31pt] (x_ijb) {$\chi^{ij\setminus m}_{C,1}$};
      %\node [factor, right=of x1, label={$f(x_2|x_1)$}] (f1) {};
     % \node [latent, right=of f1, xshift=-0.55cm] (x2) {$x_2$};
      \node [factor, between=x_Lb and x_imb ,label=$f^{i,1}_{1}$] (yi11b) {};
      \node [factor, between=x_Lb and x_ijmb ,label=$f^{i,2}_{1}$] (yi21b) {};
      \node [factor, between=x_Lb and x_ijb ,label=$f^{i,3}_{1}$] (yi31b) {};
     
      \node [factor, between=x_imb and x_ijmb ,label=right:$f^{im}_1$] (f_im) {};
      \node [factor, between=x_ijb and x_ijmb ,label=right:$f^{ij}_1$] (f_ij) {};
     
     \node [factor, right=of x_imb,  label={$f^{im\setminus j}_{2|1}$}] (f2_im) {};
      \node [latent, right=of f2_im, xshift=-0.55cm, minimum size=31pt] (x2_imb) {$\chi^{im\setminus j}_{C,2}$};
      
      \node [factor, right=of x_ijmb,   label={$f^{ijm}_{2|1}$}] (f2_ijm) {};
      \node [latent, right=of f2_ijm, xshift=-0.55cm, minimum size=31pt] (x2_ijmb) {$\chi^{ijm}_{C,2}$};
      
      \node [factor, right=of x_ijb,   label={$f^{ij\setminus m}_{2|1}$}] (f2_ij) {};
      \node [latent, right=of f2_ij, xshift=-0.55cm, minimum size=31pt] (x2_ijb) {$\chi^{ij\setminus m}_{C,2}$};
      
     
  \end{scope}
  
 \graph {
    (import nodes);
   
    % dynamic
    {x_im,x_L}--yi11, 
    {x_ijm,x_L}--yi21,  
    {x_ij,x_L}--yi31,
    %{s3,x3}--f2, s4--[dashed]f2,
   
   % (b)
    {x_imb,x_Lb}--yi11b, 
    {x_ijmb,x_Lb}--yi21b,  
    {x_ijb,x_Lb}--yi31b,
    {x_ijb,x_ijmb}--f_ij,
    {x_imb,x_ijmb}--f_im,
    {x2_ijb,x_ijb}--f2_ij,
    {x2_imb,x_imb}--f2_im,
    {x2_ijmb,x_ijmb}--f2_ijm
    };
    
\end{tikzpicture}
\caption{Robot $i$'s perspective: factor graph representing the pdf over robot $i$'s variables of interest. (a) graph before fusion. (b) graph after first fusion episode including prediction of next time step.}
      \label{fig:problemStatement}
\end{figure}
